An Empirical Analysis on the Use and Reporting of National Security Letters

Government investigatory and surveillance powers are important tools for examining crime and protecting public safety. However, since these tools must be employed in secret, it can be challenging to identify abuses or changes in use that could be of significant public interest. In this paper, we evaluate this phenomenon in the context of National Security Letters (NSLs). NSLs are a form of legal process that empowers parts of the United States federal government to request certain pieces of information for national security purposes. After initial concerns about the lack of public oversight, Congress worked to increase transparency by mandating government agencies to publish aggregated statistics on the NSL usage and by allowing the private sector to report information on NSLs in transparency reports. The implicit goal is that these transparency mechanisms should deter large-scale abuse by making it visible. We evaluate how well these mechanisms work by carefully analyzing the full range of publicly available data related to NSL use. Our findings suggest that they may not lead to the desired public scrutiny as we find published information requires significant manual effort to collect and parse data due to the lack of structure and context. Moreover, we discovered mistakes (subsequently fixed after our reporting to the ODNI), which suggests a lack of active auditing. Taken together, our case study of NSLs provides insights and suggestions for the successful construction of transparency mechanisms that enable effective public auditing.

==> bg_long.tex <==
\section{NSL: A Brief Background}\label{sec:nsl_history}

Currently, five statutory provisions authorize government agencies to issue NSLs: the Right to Financial Privacy Act (RFPA)~\cite{law:USC-12-Chapter-35-RFPA}; the Electronic Communications Privacy Act (ECPA)~\cite{law:USC-18-2701-ECPA-access-stored-communications}; the National Security Act (NSA)~\cite{law:PL-80-253-NSA}; the Fair Credit Reporting Act~\cite{law:USC-15-1681u-FCRA}; and the USA PATRIOT Act~\cite{law:PL-107-56-PATRIOT} (the last of which being the first to codify the term ``National Security Letter'' explicitly).   

% In this section, we start by giving a short overview of these five NSL statutes, followed by a summary of efforts to improve transparency around the use of NSLs (notably two amendments to the five NSL statutes that introduced reporting mandates).  
We give an overview of these statutes and efforts to improve transparency around the use of NSLs.
% (notably two amendments to the five NSL statutes that introduced reporting mandates).  
%We refer the interested reader to \Cref{sec:full_background} for a more extensive historic background on NSLs.

\subsection{The Five NSL Statutes}
The Right to Financial Privacy Act (RFPA)~\cite{law:USC-12-Chapter-35-RFPA} was the first statute used to introduce NSL authorities.  
As part of a 1986 amendment, the FBI was granted the right to request access to business records from financial institutions (amended in 2003 to include a  broader range of organizations).  
During the same period of time, the second NSL-granting statute, the Electronic Communications Privacy Act (ECPA)~\cite{law:USC-18-2701-ECPA-access-stored-communications} was enacted.
It provided access (via 18 U.S.C~\S~2709) to business records (i.e., name, address, length of service, and toll records) of wire or electronic communication service providers for counterintelligence purposes. 

In the 1990s, two more statutes were enacted granting further NSL authorities.
In 1994, the National Security Act (NSA) was amended to include a procedure for any authorized agency to request a broad array of business records from various organizations for investigating potential document leaks from government employees (codified at 50 U.S.C~\S~3162~\cite{law:USC-50-3162-codified-IAA}).
Later in 1996, the Fair Credit Reporting Act (FCRA) was amended to incorporate the fourth statutory provision for NSLs, which authorized the FBI to access credit agency records in service of national security investigations.

Finally, the PATRIOT Act~\cite{law:PL-107-56-PATRIOT} is the fifth and last NSL-granting statute, which was enacted in 2001 as a response to the terrorist attacks of September 11~\cite{wikipedia:patriot-sept-11}.
Through amending FCRA, the PATRIOT Act introduced a new procedure for government agencies to access consumer reports from credit report agencies for counterintelligence and counterterrorism investigations.
In addition, it made substantial amendments to three of the four existing NSL statutes (RFPA, ECPA, and FCRA), expanding the scope of NSLs and simplifying the administrative approval requirements.  

% In addition to providing access to sensitive records from an array of private sector institutions, the five NSL statutes initially had no mandatory judicial review, indefinite nondisclosure mandates, and few reporting requirements, making NSLs a powerful tool with limited supervision.  Due to concerns from courts and the public, various efforts have been made to increase the transparency of NSL usage and congressional oversight by introducing reporting mandates and weakening nondisclosure requirements, which we discuss below.
The five NSL statutes initially had no mandatory judicial review, indefinite nondisclosure mandates, and few reporting requirements, making NSLs a powerful tool with limited supervision.  Due to concerns from courts and the public, efforts have been made to increase the transparency and oversight of NSL usage by introducing reporting mandates and weakening nondisclosure requirements, which we discuss below.

\subsection{Subsequent Amendments}
\todo{2.2 and 2.3 can likely be combined, lots of repeated information}
% While the five NSL statutes continue to get amended in subsequent statutes, no new NSL statute was introduced after 2001.
While the five NSL statutes continue to get amended, no new NSL statute was introduced after 2001.
We briefly survey important amendments to the five existing NSL statutes after 2001.


\subsubsection{RFPA amendment in 2003}
In 2003, as part of the Intelligence Authorization Act for Fiscal Year 2004~\cite{law:PL-108-177-PATRIOT-section-374}, Congress amended the definition of financial institutions in RFPA to include a much broader range of organizations such as insurance companies and travel agencies.


\subsubsection{PATRIOT Act amendments} 
In 2006,  the 109\textsuperscript{th} Congress amended the USA PATRIOT Act with two statutes, partially as a response to earlier judicial reactions to the USA PATRIOT Act~\cite{nieland2006national}.
Specifically, two court cases \DoeVGonzales~\cite{case:DoeVGonzales} and \DoeVAshcroft~\cite{case:DoeVAshford}\footnote{
  The name ``John Doe'' is used in both cases because the gag order prohibited the disclosure of the plaintiff's identity.   
} raised First and Fourth Amendment issues with NSLs connected to the non-disclosure provisions and the absence of judicial oversight~\cite{CRS:legalBackground}. 
In the case of \DoeVAshcroft, the district court held that NSLs violated the Fourth Amendment because they authorized ``coercive searches effectively immune from any judicial process''~\cite{case:DoeVAshford:506}.
Moreover, the court held that the nondisclosure provisions unconstitutionally restrict free speech as they can prohibit disclosure without providing judicial means to challenge a ban or achieve eventual relief~\cite{case:DoeVAshford:506,case:DoeVAshford:476}.


As a reaction to both cases, while \DoeVAshcroft~was on appeal in the Second Circuit, the 109\textsuperscript{th} Congress amended the USA PATRIOT Act with the USA PATRIOT Improvement and Reauthorization Act~\cite{law:PL-109-177-PATRIOT-2005} and the USA PATRIOT Act Reauthorization Amendments Act~\cite{law:PL-109-178-PATRIOT-2005}.
Collectively, besides adding penalties for non-compliance with NSLs or their nondisclosure requirements~\cite{law:PATRIOT:amendment:3511,law:PATRIOT:amendment:1510}, these two statutes introduced judicial review on the use of NSLs and weakened the nondisclosure requirements.
Specifically, the amendments require that the Foreign Intelligence Surveillance Court (FISC) approves NSL requests and adds control mechanisms and a process to ease nondisclosure provisions~\cite{law:PATRIOT:amendment:3511,law:PATRIOT:amendment:1510}.
% Furthermore, Congress added 
%
% Miro: the following is already discussed in the next section
% Furthermore, the changes mandated classified semiannual reports about the use of NSLs to Congress and nonclassified annual statistics reports~\cite{law:PL-109-177-PATRIOT-2005-section-128}.
% The latter reports are one of the main data sources for this paper.
Regarding \DoeVAshcroft, the Second Circuit ruled in 2008 that the FBI needs to certify that disclosure of an NSL would lead to statutorily enumerated harms to justify non-disclosure provisions~\cite{case:DoeVMukasey}. Last, the amendments call for an audit on use of the NSLs from the Office of the Inspector General (referred to as the OIG reports).


\subsubsection{USA FREEDOM Act}
In 2015, Congress enacted the USA FREEDOM Act~\cite{law:PL-114-23-FREEDOM}, which revised the nondisclosure requirement, introduced an additional reporting requirement, and expressly limited the use of NSLs to specifically identify information. 
Notably, the additional reporting requirement and restrictions on the use of NSLs were direct responses to the bulk metadata collection practice of the NSA~\cite{business-records-ig-review}. 


% As an example, the original RFPA and ECPA both prohibited the disclosure of NSLs 
% included 

% various data

% Together, the five statutes enabled government agencies to use NSLs to access sensitive records from a broad array of institutions. However, despite being a power tool, the five NSLs statutes initially had no judicial oversight, strict nondisclosure mandates, and little reporting requirements, raising 

% made NSL a powerful tool for . However, despite such broad access

%It made substantial amendments to three of the four existing NSL statutes (RFPA, ECPA, and FCRA) and added a fifth one.
% The amendments in this act extended the scope of NSLs to allow the FBI to request information for people who are not themselves a foreign power or its agent but are relevant to an investigation concerning international terrorism or foreign spying.
% In addition to making NSLs more widely applicable, the amendments also simplified the approval process by authorizing Special Agents in Charge (SAC) to issue NSLs in addition to officials in the FBI headquarters~\cite{CRS:legalBackground}.

% The fifth NSL statute was introduced by amending FCRA (codified at 15~U.S.C.~\S~1681v~\cite{law:USC-15-1681-FCRA}), allowing government agencies to access consumer reports from credit reporting agencies to conduct the investigations of intelligence or terrorist activities.
% Compared to other statutes, this fifth one came with a nondisclosure requirement but not a reporting mandate (such an obligation was later added as part of a subsequent amendment).



% As part of the amendment was a nondisclosure mandate without a specific end date.\alex{maybe add a cite}






% authorized government agencies to reques

% Besides affirmatively authorizing the FBI access to various records, both statutes came with strict nondisclosure requirements (colloquially known as the ``gag order'').\footnote{An example is ``No financial institution, or officer, employee, or agent of such institution, shall disclose to any person that the Federal Bureau of Investigation has sought or obtained access to a customer's or entity's financial records under this paragraph.'' (12 U.S.C. 3414, 1986 \textit{ed.}).}



% Both the communications provider section and the Right to Financial Privacy Act section contained nondisclosure provisions8 and limitations on further dissemination except pursuant of guidelines promulgated by the Attorney General.9 Neither had an express enforcement mechanism nor identified penalties for failure to comply with either the NSL or the nondisclosure instruction.


\subsection{Reporting and Nondisclosure Mandates of NSLs}
Initially, the five NSL statutes had no mandatory judicial review, relaxed reporting requirements, and strict nondisclosure mandates\footnote{%
    As an example, the original ECPA and FCRA both prohibited the disclosure to any person.
}.
Given the broad range of data accessible via NSLs, this has unsurprisingly sparked concerns both in the public and, in response to challenges, the courts~\cite{CRS:legalBackground}. 
Over time, partially fueled by unfavorable judicial reactions (e.g., \DoeVGonzales~\cite{case:DoeVGonzales}) and various public events (e.g., the Snowden disclosures in 2013~\cite{guardian-snowden}), several efforts have been made to increase the transparency of NSL usage~\cite{schrop2017your, CRS:legalBackground}.
We highlight the two legislative efforts that are most relevant to this paper.

In 2006, Congress amended the NSL statutes with the USA PATRIOT Improvement and Reauthorization Act~\cite{law:PL-109-177-PATRIOT-2005} and the USA PATRIOT Act Reauthorization Amendments Act~\cite{law:PL-109-178-PATRIOT-2005}.
% , establishing a process for judicial review, weakening nondisclosure requirements, and introducing additional reporting requirements.
Notably, the USA PATRIOT Improvement and Reauthorization Act added two \emph{unclassified} reporting requirements. 
Section 119 of the Act initiated an audit by the Office of Inspector General of the Department of Justice to report NSL usage to Congress (``the OIG reports''). However, these reports were each singular occurrences, and the OIG is not expected to publish any further reports unless there is another mandate from Congress.
Second, Section 118 required the Attorney General of the Department of Justice to submit annual unclassified statistics about NSLs targeting \emph{US persons} to Congress~\cite{law:PL-109-177-PATRIOT-2005-section-128}.
These statistics are published as part of the Foreign Intelligence Surveillance Act reports, hence referred to as ``FISA reports''.
%Space saving measure:
%Both reports are important data sources for this paper.

In 2015, the USA FREEDOM Act~\cite{law:PL-114-23-FREEDOM} mandated additional reporting, and expressly limited the use of NSLs for explicitly specified information.
% Another victim of space saving:
% \footnote{%
%     The additional reporting requirement and restrictions on the use of NSLs are direct responses to the prior bulk metadata collection practice of the NSA~\cite{business-records-ig-review}.
% }
Notably, it mandates that the Office of the Director of National Intelligence (ODNI) should publish a report that details both the number of NSLs issued, and the number of requests for information contained in those NSLs for the past year (in addition to the FISA reports)~\cite{law:PL-114-23-FREEDOM}.
This is published as part of the National Intelligence's Annual Statistical Transparency Report (ASTR). 

Finally, in addition to adding reporting mandates and limiting the scope of NSLs, the USA FREEDOM Act introduced three major changes that relaxed the nondisclosure requirements. First, it allowed companies to report the total number of NSLs received (and customers covered by those NSLs) quantized into bands of 250, 500 or 1000.\footnote{%
    Public records~\cite{CRS:legalBackground, law:HRep-114-109} suggested that this part of the USA Freedom Act was inspired by the pre-existing voluntary agreement reached in 2014 between several technology companies and the DOJ~\cite{dojagreement:2014}.
}
In practice, a range of companies (particularly in the technology and communications sectors) take advantage of this permission and publish a rough estimate of the number of NSLs they receive as part of their annual transparency reports. We refer to such reports collectively as ``transparency reports''. Moreover, the USA FREEDOM Act codified a procedure (18 U.S.C.~\S~3511) that allows companies to request judicial review of the nondisclosure orders (commonly known as ``reciprocal notice''). Lastly, it required the Attorney General to adopt procedures to review nondisclosure orders at appropriate intervals. If disclosure is no longer believed to lead to harms listed in 18 U.S.C.~\S~2709(c)\cite{law:USC-18-2709-ECPA-access-to-records}, then the FBI should terminate the nondisclosure order and notify the company. 
% Both the second and third change may lead to potential lifting of nondisclosure requirements of certain NSLs. 
Some companies additionally publish the content of such NSLs (i.e., after the termination of nondisclosure requirements) which can provide useful metadata for analyzing past NSL issuance. We refer to such publications collectively as ``company NSLs''.

%Two procedures may  (colloquially, ``gag orders'')~\cite{fbi:term-procedures}.
% The USA FREEDOM Act mandates the FBI to review orders at appropriate intervals~\cite{law:PL-114-23-FREEDOM}.
 
%In addition to this termination procedure, companies may also use the reciprocal notice procedure to request a reassessment of the gag order.

In summary, three types of NSL reports are currently available to the public: 
\begin{itemize}
    \item OIG, FISA and ASTR reports (collectively referred to as ``Government Reports'' in Section~\ref{subsec:gov_stats}) mandated by the USA PATRIOT Improvement and Reauthorization Act and USA FREEDOM Act
    \item Company transparency reports that include the number of received NSLs
    \item NSLs disclosed by companies after the NSL's nondisclosure requirement is lifted
\end{itemize}
Understanding what the public can learn from these publicly available NSL reports, how useful the information is to the public, and the limitations of each data source is the central focus of our work.

% Besides the two major legislative efforts mentioned above, privacy companies (e.g., Google and Facebook) also actively fought for the right to inform their customers on the number of NSL requests they received. In 2014, upon reaching an agreement with the DOJ~\cite{}, 

==> old/background_miro.tex <==
\section{Background}\label{subsection:background}

The legal authority of the government to issue NSLs is rooted in five federal statutes.
Congress introduced NSLs in an amendment to the Rights to Financial Privacy Act (RFPA)~\cite{law:RFPA} to ensure that privacy laws do not prohibit financial institutions from cooperating with the FBI in foreign intelligence cases~\cite{CRS:legalBackground}.
Simultaneously, the Electronic Communications Privacy Act (ECPA)~\cite{law:ECPA} included comparable provisions for customer data of telephone companies and communications service providers.
However, NSLs under these statutes were rarely used due to two severe limitations: 
first, the target needs to be a foreign power or its agent~\cite{law:ECPA,law:RFPA:foreignAgents}.
Second, compliance was essentially voluntary since neither RFPA nor ECPA provided enforcement mechanisms.

In the 1990s, two more provisions expanded the scope of NSLs and allowed the government to use NSLs for investigations under the National Security Act~\cite{law:NSA} (leaks of classified data) and to get credit agency records under the Fair Credit Reporting Act (FCRA)~\cite{law:FCRA}.
However, NSLs remained a hardly effective and thus rarely used capability for the government.

More significant changes were introduced by the USA PATRIOT Act~\cite{law:PATRIOT} in 2001, which amended the RFPA, ECPA, and FCRA.
These changes allowed the government to request information for persons who are not themselves a foreign power or its agent but are relevant to an investigation concerning international terrorism or foreign spying.~\cite{CRS:legalBackground}
In addition to making NSLs more widely usable, the amendments also simplified the approval process by authorizing Special Agents in Charge (SAC) to issue NSLs in addition to officials in the FBI headquarters.
Furthermore, the USA PATRIOT Act added a fifth NSL section to FCRA~\cite{law:PATRIOT:sac} which allowed other government agencies than the FBI to also issue NSLs in connection to international terrorism.

The \DoeVAshcroft~\cite{case:DoeVAshford} and \DoeVGonzales~\cite{case:DoeVGonzales} cases\footnote{
  The plaintiff's name ``John Doe'' is used in both cases because the gag order prohibited the disclosure of the plaintiff's identity.   
} raised First and Fourth Amendment issues with NSLs connected to the non-disclosure provisions and the absence of judicial oversight.
The district court held that NSLs violated the Fourth Amendment because they authorize ``coercive searches effectively immune from any judicial process''~\cite{case:DoeVAshford:506}.
Moreover, the non-disclosure provisions unconstitutionally restrict free speech as they can prohibit disclosure without providing judicial means to challenge a ban or achieve eventual relief\cite{case:DoeVAshford:506,case:DoeVAshford:476}.
As a reaction to this case, and while \DoeVAshcroft was on appeal at the Second Circuit, the 109\textsuperscript{th} Congress amended the USA PATRIOT Act.
The amendments require that the Foreign Intelligence Surveillance Court (FISC) approves NSL requests and adds control mechanisms and a process to ease non-disclosure provisions\cite{law:PATRIOT:amendment:3511,law:PATRIOT:amendment:1510}.
Furthermore, Congress added penalties for non-compliance with NSLs or their non-disclosure requirements~\cite{law:PATRIOT:amendment:3511,law:PATRIOT:amendment:1510}.
Finally, the changes mandated classified semiannual reports about the use of NSLs to Congress and nonclassified annual statistics~\cite{law:PATRIOT:congress}.
The latter reports are one of our main data sources for this paper.
Regarding \DoeVAshcroft, the Second Circuit ruled in 2008 that the FBI needs to certify that disclosure of an NSL would lead to statutorily enumerated harms to justify non-disclosure provisions~\cite{case:DoeVMukasey}.

After the USA PATRIOT Improvement and Reauthorization Act in 2006, the NSLs became an effective tool for the government (predominantly the FBI).
They can now be used to request information pertaining to individuals relevant to foreign intelligence cases from financial institutions, telephone companies, communication providers, and credit agencies.
The NSLs are enforceable and failure to comply can be penalized.
Furthermore, a non-disclosure provision can be attached to NSLs to avoid jeopardizing ongoing investigations.
To ensure commensurability, Congress added the requirements that the FISC approves NSLs as well as enforces limits on the permissible non-disclosure scope.

